CrySL: Validating Correct Usage of Cryptographic APIs

Various studies have empirically shown that the majority of Java and Android apps misuse cryptographic libraries, causing devastating breaches of data security. Therefore, it is crucial to detect such misuses early in the development process. The fact that insecure usages are not the exception but the norm precludes approaches based on property inference and anomaly detection. In this paper, we present CrySL, a definition language that enables cryptography experts to specify the secure usage of the cryptographic libraries that they provide. CrySL combines the generic concepts of method-call sequences and data-flow constraints with domain-specific constraints related to cryptographic algorithms and their parameters. We have implemented a compiler that translates a CrySL ruleset into a context- and flow-sensitive demand-driven static analysis. The analysis automatically checks a given Java or Android app for violations of the CrySL-encoded rules. We empirically evaluated our ruleset through analyzing 10,001 Android apps. Our results show that misuse of cryptographic APIs is still widespread, with 96% of apps containing at least one misuse. However, we observed fewer of the misuses that were reported in previous work.

==> algorithms/crysl-events-semantics.tex <==
\begin{figure}
\small
\begin{algorithmic}
\State e$_1$, e$_2$ := Event e$_1$ must occur before event e$_2$
\State e$_1$ $|$ e$_2$ := Exactly one of the two events e$_1$ and e$_2$ must occur
\State e? := Event e is optional
\State e+ := Event e must at least occur once
\end{algorithmic}

\caption{Semantics of Event Order Syntax in \DSL.}
\label{def:EO}
\end{figure}

==> figures/algorithm.tex <==
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\INPUT{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\OUTPUT{\item[\algorithmicoutput]}
\begin{algorithm}
  \caption{Compute objects that are not used in compliance to a set of rules.}
  \begin{algorithmic}[1]
		\INPUT{Set of \DSL rules $\mathcal{R}$}
		\OUTPUT{Set of objects $\{o \in \allocs \mid \sat(o,s,r) = false, r \in \mathcal{R}, s\in \stmts\}$}
    \Statex
    \Function{DoMagic}{$\mathcal{R}$}
      \State $objs \gets \{(o,r) \mid o \in \allocs,type(o) = r \in \mathcal{R}\}$ 
      \State $\objState \gets \emptyset$ 
      \State $\objEnv \gets \emptyset$ 
      \State $res \gets \emptyset$ 
      \For{$(o,r) \in objs, s \in \stmts$}
					\State $\objState(o,s) = typestates(o,s)$
					\If{$err \in \objState(o,s)$}
						\State $res \, \cup= \{o\}$
					\EndIf
					\If{$s: o.m(vars) \wedge (m,args) \in \methods_r$}
						\For{$i \gets  1 \textrm{ to } sizeof(args)$}					
							\State $\objEnv(o,args_i) = pts\textnormal{-}to(vars_i)$
						\EndFor
					\EndIf
      \EndFor
			\For{$(o,r) \in objs, (v,f) \in  \constraint_r,u \in \objEnv(o,v)$}				
					\If{$\neg f(u)$}
							\State $res \, \cup= \{o\}$
					\EndIf
      \EndFor
      \State $\ensPreds \gets \emptyset$ 
			\While{$\ensPreds$ changes}
				\For{$(o,r) \in objs, s \in  \stmts, t\in \objState(o,s)$}
						\If{$\{(\objEnv(o,args_i),s,p) \mid (p,args)\in \reqPreds_r\} \subset \ensPreds$}
							\For{$(p,args) \in \genPreds_r(t), i \gets  1 \textrm{ to } sizeof(args)$}
									\If{$args_i = this$}
										\State $\ensPreds \cup = \{(o,s,p)\} $
									\EndIf
									\If{$args_i \neq this$}
										\State $\ensPreds \cup = \{(u,s,p) \mid u \in pts\textnormal{-}to(args_i)\} $
									\EndIf
							\EndFor
						\EndIf
      \EndFor
			\EndWhile
      \State \Return{$res$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> figures/appsmisuses.tex <==
\begin{figure}[t]
\begin{tikzpicture}[trim axis right, trim axis left]
\begin{axis}[
    symbolic x coords={MIN, Typestate Errors, Missing Predicates, Forbidden Events, Internal-Constraint Violations, MAX},
    xtick=data,
    bar width=30,
    ybar stacked,
    ytick={0, 1000, 2000, 3000, 4000},
    width=9cm,
    height=4.5cm,
    xticklabel style={text width=1.5cm,align=center},
    major x tick style = transparent,
    xmin=MIN,
    xmax=MAX  ]
    \addplot [ybar,fill=lightgray,draw=black] coordinates { (Typestate Errors, 1845) (Missing Predicates, 1222) (Forbidden Events, 2640) (Internal-Constraint Violations,4001) };
\end{axis}
\end{tikzpicture}
\caption{Number of Apps per Misuse Type}
\label{fig:misuseinApps}
\end{figure}

==> figures/overallmisuses.tex <==
%\pgfplotsset{scaled y ticks=false}
\begin{figure}[t]
\begin{tikzpicture}[trim axis right, trim axis left]
\begin{axis}[
    symbolic x coords={MIN, Typestate Errors, Missing Predicates, Forbidden Events, Internal-Constraint Violations, MAX},
    xtick=data,
    bar width=30,
    ybar stacked,
    ytick={0, 2000, 4000, 6000, 8000, 10000, 12000},
    width=9cm,
    height=4.5cm,
    xticklabel style={text width=1.5cm,align=center},
    major x tick style = transparent,
    xmin=MIN,
    xmax=MAX  ]
    \addplot [ybar,fill=lightgray,draw=black] coordinates {(Typestate Errors, 2773) (Missing Predicates, 4209) (Forbidden Events, 3466) (Internal-Constraint Violations,12229) };
\end{axis}
\end{tikzpicture}
\caption{Types of Misuses Overall \eb{Could drop figure if space needed}}
\label{fig:misusesOverall}
\end{figure}

==> tables/predicates.tex <==
\begin{table}
  \centering
  \caption{\DSL Predicates}
    \begin{tabular}{ll}
    \toprule
    \textbf{Predicate} & \textbf{Parameters} \\
    \midrule
    encrypted & ciphertext, plaintext \\
    digested & hashvalue, input \\
    macced & MAC, input \\
    generatedKey & key, algorithm \\
    keySpec & keyspec, length \\
    random & randomObject \\
    IVParam & IV \\
    generatedPubKey & key, algorithm \\
    generatedPrivKey & key, algorithm \\
    generatedKeyPair & keypair, algorithm \\
    signed & signature, signedObject \\
    verified & signature \\
    \bottomrule
    \end{tabular}%
  \label{tab:predicates}%
\end{table}%

